A Parallel Cross-Lingual Benchmark for Multimodal Idiomaticity Understanding

Potentially idiomatic expressions (PIEs) construe meanings inherently tied to the everyday experience of a given language community. As such, they constitute an interesting challenge for assessing the linguistic (and to some extent cultural) capabilities of NLP systems. In this paper, we present XMPIE, a parallel multilingual and multimodal dataset of potentially idiomatic expressions. The dataset, containing 34 languages and over ten thousand items, allows comparative analyses of idiomatic patterns among language-specific realisations and preferences in order to gather insights about shared cultural aspects. This parallel dataset allows to evaluate model performance for a given PIE in different languages and whether idiomatic understanding in one language can be transferred to another. Moreover, the dataset supports the study of PIEs across textual and visual modalities, to measure to what extent PIE understanding in one modality transfers or implies in understanding in another modality (text vs. image). The data was created by language experts, with both textual and visual components crafted under multilingual guidelines, and each PIE is accompanied by five images representing a spectrum from idiomatic to literal meanings, including semantically related and random distractors. The result is a high-quality benchmark for evaluating multilingual and multimodal idiomatic language understanding.

==> tab_examples_original.tex <==
\begin{table*}[htbp!]
\centering
\begin{tabular}{llll}
\hline
Mapping & Class                                       & Nature of Mapping                                                                                     & Examples                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline
1 - 1   & Source idiom -- Target Idiom                & Target idiom has identical or near-identical wording (lexis and/or syntactical structure) and meaning & \begin{tabular}[c]{@{}l@{}}"bad apple” --\textgreater{} çürük elma ('rotten apple', Turkish); ცუდი ნაყოფი 'c'udi naqop'i' (\`{}bad fruit', Georgian); תפוח רקוב ('rotten apple', Hebrew); maça podre ('apple rotten, Brazilian Portuguese)\\"add fuel to the fire” --\textgreater{} yangına körükle gitmek ('to go to the fire with a bellows', Turkish); hælde benzin på bålet ('pour gasoline to the fire', Danish); richno ladi sti fotia ('throw oil on the fire', Modern Greek); deitar achas na fogueira ('to lie down woodsticks on the bonfire', European Portuguese); colocar lenha na fogueira ('to put woodsticks in the bonfire', Brazilian Portuguese); įpilti aliejaus į ugnį (pour oil into the fire, Lithuanian); afegir llenya al foc (add firewood to the fire, Catalan); 火上浇油 (in the fire pour oil, Chinese)\\"apples and oranges" --\textgreater{} "epler og pærer" (apples and pears, Norwegian); Äppel a Bieren (apples and pears, Luxembourgish); jabolka in hruške (apples and pears, Slovenian)\\"big fish” --\textgreater{} დიდი მოთამაშე 'didi motamashe' ('big player', Georgian)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\
        &                                             & Target idiom has different wording (lexis and/or syntactical structure) but same conceptual meaning   & \begin{tabular}[c]{@{}l@{}}"bad apple” --\textgreater{} развалена стока 'razvalena stoka' ('rotten goods', Bulgarian)\\ "eager beaver" --\textgreater{}الله تان بیر گون اوغورلامیش /Allahtan bir gün oğurlamış ('stealing one day from God', Azeri)\\"ancient history" --\textgreater{} کهنه پالان / köhnə palan (old packsaddle, Azeri); acqua passata ('water passed', Italian)\\"chocolate teapot" --\textgreater{} emplastro numa perna de pau ('patch on a leg of wood', European Portuguese)\\"beer and skittles" --\textgreater{} تزه کوزه سرین سو/təze küzə sərin su (new clay jug, cold water, Azeri) \\"apples and oranges" --\textgreater{} "nebo i zemlja" (Ukrainian), като деня и нощта 'kato denya i noshtta' ('like day-the and night-the', Bulgarian); alhos com bugalhos ('garlics with \textit{bu}garlics', European Portuguese)\\"close shave" (noun phrase) --\textgreater{} o vlások (adverbial phrase, \`{}by a hair', Slovak); para tricha (adverbial phrase, \`{}by a hair', Modern Greek); қыл көпір 'qyl köpir' ('bridge made of hair', Kazakh)\\"heart of gold" --\textgreater{} obi sara sara ('clean heart', Igbo)\\ "add fuel to the fire" --\textgreater{} آتش بیار معرکه شدن /atash biyar-e mareke shodan ('to become the fire-bringer of the battlefield', Farsi)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\
1 - 0   & Source idiom -- Target non-idiom            & Target language uses (non-idiomatic) descriptive expression or has no equivalent                      & \begin{tabular}[c]{@{}l@{}}"chocolate teapot” --\textgreater{} აბსოლუტურად უსარგებლო რამ 'absoluturad usargeblo ram' ('absolutely useless thing', Georgian)\\"brain drain" --\textgreater{} فرار مغزها/farar-e maghzhā ('escape of brains', Farsi) \\"beauty sleep" --\textgreater{} none (Azeri); none (Farsi) \\"agony aunt” --\textgreater{} conselheiro sentimental ('counselor sentimental', European Portuguese, Brazilian Portuguese); მკითხველის მრჩეველი 'mkitʻxvelis mrčʻeveli' (' of the reader advisor', Georgian); none (Swahili); none (Hebrew); none (Azeri); none (Farsi); none (Modern Greek)\\"best man” --\textgreater{} "apoio do noivo” ('support of the groom', European Portuguese); padrinho de casamento ('godfather of wedding', European Portuguese; Brazilian Portuguese); دولہے کا سہارا (the groom's support, Urdu); none (Norwegian); none (Chinese)\\"cloud nine” --\textgreater{} bulutların üzerinde (Turkish) \\"bear market” --\textgreater{} none (Turkish); \\"devil’s advocate” 'anayejumuika' ('the one who participates/joins', Swahili), 'mpinzani wa makusudi' ('a deliberate opponent', Swahili), 'mjadala wa kupinga' ('argumentative for discussion', Swahili)\\"baby blue" --\textgreater{} depressió postpart ('depression postbirth', Catalan), depressão pós-parto ('depression postbirth' European Portuguese, Brazilian Portuguese), следродилна депресия 'sledrodilna depresiya' ('afterbirth depression', Bulgarian); gyermekágyi lehangoltság ('afterbirth depression', Hungarian)\\"busman's holiday" --\textgreater{} none (European Portuguese)\\"cat's eye" --\textgreater{} none (Uzbek); none (Latvian)\end{tabular}                                                                                                                                                                \\
        &                                             & Target language uses an idiom made up of single lexical item (not an MWE)                             & \begin{tabular}[c]{@{}l@{}}"brain teaser” --\textgreater{} "pazli” (Georgian); "nøtt" (nut, Norwegian) \\"busy bee” --\textgreater{} "futkari” (Georgian)\\ "brain teaser" --\textgreater{} تاپپاجا/tappaca (Azeri), "brain teaser" --\textgreater{} معما / moamma (Farsi) \\"cheat sheet" --\textgreater{} cola (Brazilian Portuguese); skonaki (Modern Greek), пищов 'pishtov' (Bulgarian); puska (Hungarian)\\"blind alley" --\textgreater{} "akligatvis" (Lithuanian)\\"eager beaver" --\textgreater{} včelička (little bee, Slovak)\\black box" --\textgreater{} fumbo (mystery, Swahili)\\"can of worms" --\textgreater{} "vespaio" (Italian) \\"chicken feed" --\textgreater{} drobtinice (breadcrumbs, Slovenian); "chicken feed" --\textgreater{} shịshị (Igbo)\\"brass neck" -\textgreater{} ڈھٹائی (Urdu; meaning: shamelessness)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\
1 - N   & Source idiom -- multiple Target idiom       & Source idiom has multiple Target idioms                                                               & \begin{tabular}[c]{@{}l@{}}"brownie points” --\textgreater{} "jó pont” or "pirospont” (Hungarian)\\"brain drain" --\textgreater{} "protų nutekėjimas", "smegenų nutekėjimas" (Lithuanian)\\"blind alley" --\textgreater{} به ترکستان رفتن/be Torkestan raftan (to go to Turkestan, Farsi), آب در هاون کوبیدن /ab dar havan kubidan (pounding water in a mortar, Farsi)\\"apples and oranges" --\textgreater{} بیرگازانا آتسان قینمز /bir gazana atsan geynəməz (not to boil if you put [them] in one cauldron, Azeri), الله لاری فرق المخ /Allahları fərq eləməx (to have different Gods, Azeri)\\"can of worms'' --\textgreater{} ninho de vespas, caixa de marimbondos, caixa de Pandora (Brazilian Portuguese)\\"chocolate teapot" --\textgreater{} "jak p'jate koleso do voza", "jak sobaci p'jata noha", "marna robota" (Ukrainian)\\"cloud nine" --\textgreater{} ברקיע השביעי, מאושר עד הגג (Hebrew); "ancient history" --\textgreater{} histórias antigas, águas passadas (European Portuguese)\\"bleeding heart" --\textgreater{} coração de manteiga, coração mole (European Portuguese)\\"apples and oranges" --\textgreater{} kruške i jabuke, babe i žabe (Serbian)\\"can of worms" --\textgreater{} отварање на пандорината кутија, не отварај рана (Macedonian)\\"big fish" --\textgreater{} mtu mkubwa, mtu muhimu (Swahili)\\"black market" -\textgreater{} черен пазар 'cheren pazar', черн борса 'cherna borsa' (Bulgarian)\\"brass neck" -\textgreater{} арсыз/бетсыз arsyz/betsyz, faceless, Kazakh)\\"piece of cake" --\textgreater{} ~проще~пареной~репы; раз плюнуть; плевая работа; как дважды два; что два пальца об асфальт (Russian)\\"blame game" --\textgreater{} искать козла отпущения; вешать собак (Russian)\\"piece of cake" --\textgreater{} xamirqan qil sug'urganday, og'zining yeli (Uzbek)\end{tabular}  \\
N - 1   & Multiple source idioms -- same Target idiom & Multiple source idioms have same Target idiom                                                         & \begin{tabular}[c]{@{}l@{}}"big fish" and "big cheese" --\textgreater{} "peix gros” (Catalan); "didelė žuvis” (Lithuanian); "veľké zviera" (Slovak); بویوک باش/böyük baş (Azeri)\\"big cheese", "big wig", "big fish" -\textgreater{} важна клечка 'vazhna klechka' (Bulgarian); stor kanon (Danish); "کله گنده / kalle gonde" (Farsi); "oke osisi” (big tree, Igbo) \\"big fish", "big cheese" and "big wig" --\textgreater{} "Važna osoba" (Ukrainian); "velika živina" (Slovenian)\\"big wig" and "big cheese” --\textgreater{} "大人物” (Chinese); "liels čiekurs" (Latvian); большая шишка (Russian); katta odam (Uzbek) \\"blind alley" and "brick wall" --\textgreater{} מבוי סתום (Hebrew)\\"eager beaver" and "busy bee" --\textgreater{} "vredan kao pčela" (Serbian); "vreden kao pčela/mravka" (Macedonian)\\ "dead end" and "blind alley" --\textgreater{} Sakgaass (sack alley, Luxembourgish)\\"close call" and "close shave" --\textgreater{} kuponea chupuchupu (Swahili) \\"close shave" and "close call" --\textgreater{} "per un pelo" (Italian); på et hængende hår (Danish); اینه نین اوجوجا /iynənin ucuca (Azeri) \\"meat and potatoes" and "bread and butter" --\textgreater{} arroz e feijão (Brazilian Portuguese)\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         
\hline
\end{tabular}
\caption{Cross-linguistic mappings of English idioms showing different types of equivalence and adaptation.}
\label{tab:idiom-mappings}
\end{table*}
